QUIC-EST: A Transmission Scheme to Maximize VoI of Multi-Stream Correlated Data Flows

New advanced applications, such as autonomous driving and haptic communication, require to transmit multi-sensory data and require low latency and high reliability. These applications include. Existing implementations for such services have mostly relied on ad hoc scheduling and send rate adaptation mechanisms, implemented directly by the application and running over UDP. In this work, we propose a transmission scheme that relies on the features of the recently developed QUIC transport protocol, providing reliability where needed, and standardized congestion control, without compromising latency. Furthermore, we propose a scheduler for sensor data transmissions on the transport layer that can exploit the correlations over time and across sensors. This mechanism allows applications to maximize the Value of Information (VoI) of the transmitted data, as we demonstrate through simulations in two realistic application scenarios.

==> tactile.tex <==

\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\scriptsize}}
\tikzstyle{dotted}= [dash pattern=on \pgflinewidth off 0.5mm] 
\tikzstyle{dashed}= [dash pattern=on 7.5*0.8*0.8pt off 7.5*0.4*0.8pt]
\tikzstyle{dashdotted} = [dash pattern=on 7.5*0.8*0.6pt off 7.5*0.8*0.3pt on \the\pgflinewidth off 7.5*0.8*0.3pt]
\tikzstyle{dotted2} = [dash pattern=on 7.5*0.8*0.3pt off 7.5*0.8*0.2pt]


\begin{axis}[%
width=\fwidth,
height=\fheight,
at={(0,0)},
scale only axis,
xmin=250,
xmax=1250,
xlabel near ticks,
xlabel style={font=\footnotesize\color{white!15!black}},
ylabel near ticks,
ymin=0.75,
ymax=1,
ylabel style={font=\footnotesize\color{white!15!black}},
ylabel={Normalized \gls{qoe}},
xlabel={Capacity (kbps)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
% legend style={font=\scriptsize, at={(0.23,0.91)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black}
legend style={font=\scriptsize, at={(0.975,0.05)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=orange_D, dashdotted, line width=1pt]
  table[row sep=crcr]{
250	0.811327160704771\\
375	0.873073430858262\\
500	0.906642294924310\\
625	0.928478513613372\\
750	0.944523237335027\\
875	0.957333465347718\\
1000	0.968317577713290\\
1125	0.978513150627807\\
1250	0.988146714349142\\
};
\addlegendentry{FIFO}


\addplot [color=cyan, line width=0.8pt, mark size=1.5pt, mark=*, mark options={solid, fill=cyan, cyan}]
  table[row sep=crcr]{
250	0.811327160704771\\
375	0.873073430858262\\
500	0.906642294924310\\
625	0.928478513613372\\
750	0.944523237335027\\
875	0.957333465347718\\
1000	0.968317577713290\\
1125	0.978513150627807\\
1250	0.988146714349142\\
};
\addlegendentry{VoI-based}

\addplot [color=violet, dashed, line width=0.8pt]
  table[row sep=crcr]{
250	0.811327160704771\\
375	0.873073430858262\\
500	0.906642294924310\\
625	0.928478513613372\\
750	0.944523237335027\\
875	0.957333465347718\\
1000	0.968317577713290\\
1125	0.978513150627807\\
1250	0.988146714349142\\
};
\addlegendentry{Cross-sensor VoI}


\addplot [color=black, dotted, line width=1pt]
  table[row sep=crcr]{
250	0.926166638525475\\
375	0.993308958804284\\
500	0.999576044787255\\
625	0.999957237148134\\
750	0.999992927914319\\
875	0.999998484559529\\
1000	0.999999627415448\\
1125	0.999999903704258\\
1250	0.999999977494089\\
  };
\addlegendentry{QUIC-EST}

\end{axis}
\end{tikzpicture}


==> v2x-one.tex <==
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\scriptsize}}
\tikzstyle{dotted}= [dash pattern=on \pgflinewidth off 0.5mm] 
\tikzstyle{dashed}= [dash pattern=on 7.5*0.8*0.8pt off 7.5*0.4*0.8pt]
\tikzstyle{dashdotted} = [dash pattern=on 7.5*0.8*0.6pt off 7.5*0.8*0.3pt on \the\pgflinewidth off 7.5*0.8*0.3pt]
\tikzstyle{dotted2} = [dash pattern=on 7.5*0.8*0.3pt off 7.5*0.8*0.2pt]


\begin{axis}[%
width=\fwidth,
height=\fheight,
at={(0,0)},
scale only axis,
xmin=20,
xmax=120,
xlabel near ticks,
xlabel style={font=\footnotesize\color{white!15!black}},
ylabel near ticks,
ymin=0,
ymax=1,
ylabel style={font=\footnotesize\color{white!15!black}},
ylabel={Normalized \gls{voi}},
xlabel={Capacity (Mbps)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
% legend style={font=\scriptsize, at={(0.23,0.91)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black}
legend style={font=\scriptsize, at={(0.5,1.2)},anchor=north, legend cell align=left, align=left, draw=white!15!black,legend columns=-1}
]

\addplot [color=orange_D, dashdotted, line width=0.8pt]
  table[row sep=crcr]{
20	0.0821828800000001\\
25	0.100501120000000\\
30	0.124643360000000\\
35	0.141500480000000\\
40	0.167696320000000\\
45	0.187472800000000\\
50	0.212070080000000\\
55	0.229869600000000\\
60	0.254791840000000\\
65	0.277067680000000\\
70	0.300326400000000\\
75	0.323084960000000\\
80	0.349790560000000\\
85	0.362538400000000\\
90	0.389626560000000\\
95	0.408533280000000\\
100	0.437361440000000\\
105	0.457106080000000\\
110	0.476614080000000\\
115	0.502749599999999\\
120	0.523282240000000\\
};
\addlegendentry{FIFO}



\addplot [color=cyan, line width=0.8pt, mark size=1.5pt, mark=*, mark options={solid, fill=cyan, cyan}]
  table[row sep=crcr]{
20	0.0769862400000011\\
25	0.0930411200000008\\
30	0.124468320000000\\
35	0.157482560000000\\
40	0.169913440000000\\
45	0.203078400000000\\
50	0.233169760000001\\
55	0.254150720000001\\
60	0.279463360000000\\
65	0.308903199999999\\
70	0.333814239999999\\
75	0.353992479999999\\
80	0.384332639999999\\
85	0.411545599999999\\
90	0.429812319999999\\
95	0.455355040000000\\
100	0.481854400000001\\
105	0.501951040000000\\
110	0.522933920000001\\
115	0.547256800000001\\
120	0.565069120000000\\
};
\addlegendentry{VoI-based}

\addplot [color=violet, dashed, line width=0.8pt]
  table[row sep=crcr]{
20	0.470400000000007\\
25	0.627200000000008\\
30	0.744800000000008\\
35	0.744800000000008\\
40	0.816240000000020\\
45	0.817280000000014\\
50	0.863359999999999\\
55	0.920960000000009\\
60	0.967039999999989\\
65	0.990080000000013\\
70	0.990080000000013\\
75	0.995683999999994\\
80	0.995683999999994\\
85	0.995683999999994\\
90	0.995683999999994\\
95	0.995683999999994\\
100	0.995683999999994\\
105	0.995683999999994\\
110	0.995683999999994\\
115	0.995683999999994\\
120	0.995683999999994\\
};
\addlegendentry{Cross-sensor VoI}


\addplot [color=black, dotted, line width=0.8pt]
  table[row sep=crcr]{
20	0.470142400000007\\
25	0.626942400000008\\
30	0.755731199999999\\
35	0.801921919999990\\
40	0.859593119999989\\
45	0.905684320000008\\
50	0.951764319999986\\
55	0.974838879999985\\
60	0.974884959999986\\
65	0.990080000000013\\
70	0.990080000000013\\
75	0.995696799999994\\
80	0.995696799999994\\
85	0.995696799999994\\
90	0.995696799999994\\
95	0.995696799999994\\
100	0.995696799999994\\
105	0.995696799999994\\
110	0.995696799999994\\
115	0.995696799999994\\
120	0.995696799999994\\
  };
\addlegendentry{QUIC-EST}

\end{axis}
\end{tikzpicture}

==> v2x-two.tex <==
\begin{tikzpicture} \begin{axis}
[ ybar, enlarge x limits=0.1,ylabel near ticks, ymin=0, width=\fwidth,ylabel style={font=\footnotesize\color{white!15!black}}, xlabel style={font=\footnotesize\color{white!15!black}}, height=0.5\columnwidth, bar width=0.15cm, ymax=10, anchor=north,legend columns=-1, ylabel={Scheduling frequency (Hz)}, symbolic x coords={LIDAR, Front, Back, Left, Right}, legend style={at={(0.5,1.23)},anchor=north,font=\scriptsize}, xtick=data,  x tick label style={rotate=30,anchor=east,font=\footnotesize\color{white!15!black}}, y tick label style={font=\footnotesize\color{white!15!black}}  ] 


\addplot[color=orange_D,dashdotted, fill={orange_D!50}] coordinates {(LIDAR, 6.027) (Front, 6.567) (Back, 6.588) (Left, 6.638) (Right, 6.602)};
\addplot[color=cyan, fill={cyan!50}] coordinates {(LIDAR, 5.802) (Front, 8.112) (Back, 8.142) (Left, 5.877) (Right, 5.802)};
\addplot[color=violet,dashed, fill={violet!50}] coordinates {(LIDAR, 4) (Front, 10) (Back, 10) (Left, 10) (Right, 10)};
\addplot[color=black,dotted, fill={black!50}] coordinates {(LIDAR, 4) (Front, 10) (Back, 10) (Left, 10) (Right, 10)};

\legend{FIFO, VoI-based, Cross-sensor, QUIC-EST} 

\end{axis}
\end{tikzpicture}


